Automating Control of Overestimation Bias for Reinforcement Learning

Overestimation bias control techniques are used by the majority of high-performing off-policy reinforcement learning algorithms. However, most of these techniques rely on pre-defined bias correction policies that are either not flexible enough or require environment-specific tuning of hyperparameters. In this work, we present a general data-driven approach for the automatic selection of bias control hyperparameters. We demonstrate its effectiveness on three algorithms: Truncated Quantile Critics, Weighted Delayed DDPG, and Maxmin Q-learning. The proposed technique eliminates the need for an extensive hyperparameter search. We show that it leads to a significant reduction of the actual number of interactions while preserving the performance.

==> images.tex <==
\section{Blueprint images}
Here are the plot we have and are planning to do.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{icml_images/main_exps.pdf}
\caption{
Main experiments. Single problem with Hopper, maaaybe some improvement on Walker2d, Humanoid, HumanoidBulletEnv. Maybe we should again exclude HalfCheetah.
}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{icml_images/wd3.pdf}
\caption{
AdaWD3 experiments. We have good results on Walker2dPyBullet, maybe HalfCheetah, maybe Walker2d would be somewhat non trivial. The rest look like trivial ones.
}
\end{figure}


\begin{figure}[t!]
\centering
\includegraphics[width=0.8\textwidth]{icml_images/d_to_zero.pdf}
\caption{
Almost convergence.
}
\end{figure}



==> theory_section.tex <==
\newcommand{\mct}{\mathcal{T}}
\newcommand{\mcs}{\mathcal{S}}
By $F_X(x)$ in this section we define distribution function of random variable $X$:

\begin{equation}
    F_X(x) = P(X \leq x)
\end{equation}

\textbf{Definition.} Lets define truncation operator $\mcs^\eta(\cdot), \; 0 \leq \eta < 1$ for one-dimensional random variable via distribution function of the result:

\begin{equation}
F_{\mcs^\eta(Z)}(z) =
    \begin{cases}
      \dfrac{F_Z(z)}{1-\eta}, \quad z \leq F^{-1}_Z(1 - \eta)\\
      1, \quad z > F^{-1}_Z(1 - \eta)
    \end{cases}
\end{equation}

\textbf{Definition.} We introduce non-strict partial order on space of one-dimensional random variables:
\begin{equation}
    Z_1 \preccurlyeq Z_2 \quad \text{if} \quad F_{Z_1}(z) \geq F_{Z_2}(z) \quad \forall z
\end{equation}

\begin{lemma}
$Z_1 \preccurlyeq Z_2 \Rightarrow \ex Z_1 \leq \ex Z_2$
\end{lemma}

\begin{equation}
    Z_1 \preccurlyeq Z_2 \Rightarrow F_{Z_1}(z) \geq F_{Z_2}(z) \quad \forall z \Rightarrow F^{-1}_{Z_1}(w) \leq F^{-1}_{Z_2}(w) \quad \forall w  
\end{equation}

\begin{proof}
We can rewrite the expectations in Lebesgue form:

\begin{equation}
    \ex Z_1 = \int_{0}^{1} F^{-1}_{Z_1}(w) \; dw \leq \int_{0}^{1} F^{-1}_{Z_2}(w) \; dw = \ex Z_2
\end{equation}
\end{proof}

\begin{lemma}
$\forall Z_1, Z_2, \eta: \; 0\leq \eta < 1, Z_1 \preccurlyeq Z_2 \Rightarrow \mcs^\eta Z_1 \preccurlyeq \mcs^\eta Z_2$
\end{lemma}
\begin{proof}
Let us show that by definition of $\mcs^\eta$ and order $\preccurlyeq$ the lemma holds true and $F_{\mcs^\eta(Z_1)}(z) \geq F_{\mcs^\eta(Z_2)}(z) \quad \forall z$ :

\begin{equation}
\begin{aligned}
    z \leq F^{-1}_{Z_1}(1 - \eta) &\Rightarrow \dfrac{F_{Z_1}(z)}{1-\eta} \geq \dfrac{F_{Z_2}(z)}{1-\eta}\\
    F^{-1}_{Z_1}(1 - \eta) < z \leq F^{-1}_{Z_2}(1 - \eta) &\Rightarrow 1 \geq \dfrac{F_{Z_2}(z)}{1-\eta}\\
    z > F^{-1}_{Z_2}(1 - \eta) &\Rightarrow 1 = 1
\end{aligned}
\end{equation}

It follows that $F_{\mcs^\eta(Z_1)}(z) \geq F_{\mcs^\eta(Z_2)}(z) \ \forall z$.
\end{proof}


\begin{lemma}
$\forall Z, \eta_1, \eta_2: \;\; 0 \leq \eta_1, \eta_2 < 1$, $\eta_1 \geq \eta_2 \Rightarrow \mcs^{\eta_1} Z \preccurlyeq \mcs^{\eta_2} Z$
\end{lemma}

\begin{proof}
Also by definition
\begin{equation}
\begin{aligned}
    z \leq F^{-1}_Z(1 - \eta_1) &\Rightarrow \dfrac{F_Z(z)}{1-\eta_1} \geq \dfrac{F_Z(z)}{1-\eta_2}\\
    F^{-1}_Z(1 - \eta_1) < z \leq F^{-1}_Z(1 - \eta_2) &\Rightarrow 1 \geq \dfrac{F_Z(z)}{1-\eta_2}\\
    z > F^{-1}_Z(1 - \eta_2) &\Rightarrow 1 = 1
\end{aligned}
\end{equation}
From here it follows that $\mcs^{\eta_1} Z \preccurlyeq \mcs^{\eta_2}$.
\end{proof}


\begin{lemma}
$Z_1 \preccurlyeq Z_2, \eta_1 \geq \eta_2 \Rightarrow \mcs^{\eta_1}Z_1 \preccurlyeq \mcs^{\eta_2}Z_2$
\end{lemma}

\begin{proof}
Applying previous two lemmas we get the result:
\begin{equation}
    \mcs^{\eta_1}Z_1 \preccurlyeq \mcs^{\eta_2} Z_1 \preccurlyeq \mcs^{\eta_2}Z_2
\end{equation}
\end{proof}


\begin{lemma}
$\forall Z_1, Z_2, X:\quad  X \perp Z_i, Z_1 \preccurlyeq Z_2 \Rightarrow Z_1 + X \preccurlyeq Z_2 + X$
\end{lemma}
\begin{proof}
$$Y_1 = Z_1 + X, \; Y_2 = Z_2 + X$$
\begin{equation*}
    F_{Y_1}(y) = P(Y_1 \leq y) = \int_\mathcal{X} p(x) P(Z_1 \leq y - x) \; dx = \\
\end{equation*}
\begin{equation}
    \int_\mathcal{X} p(x) F_{Z_1}(y - x) \; dx \geq  \int_\mathcal{X} p(x) F_{Z_2}(y - x) \; dx = F_{Y_2}(y)
\end{equation}
\end{proof}
Now let's consider random fields over state-action domain instead of scalar random variables. We overload notation and from here we also designate them by $Z(s,a), \quad s \in \mcs, a \in \mathcal{A}$.


\textbf{Definition.} Our partial order can be extended on random fields: 
\begin{equation}
Z_1(\cdot, \cdot) \preccurlyeq Z_2(\cdot, \cdot) \; \text{if} \; Z_1(s,a) \preccurlyeq Z_2(s,a) \quad \forall s \in \mathcal{S}, a \in \mathcal{A}.
\end{equation}

\begin{lemma}
$\forall Z_1, Z_2: \; Z_1 \preccurlyeq Z_2, \forall p(s,a) \Rightarrow \ex_{s, a \sim p} Z_1(s, a) \preccurlyeq \ex_{s, a \sim p} Z_2(s, a)$
\end{lemma}
\begin{proof}
\begin{equation}
    Y_i = \ex_{s,a \sim p} Z_i(s, a)
\end{equation}

\begin{equation}
    F_{Y_1}(y) = P(Y_1 \leq y) = \int\limits_{\mathcal{S}, \mathcal{A}} p(s,a) P(Z_1 \leq y | s, a) \; ds da \geq \int\limits_{\mathcal{S}, \mathcal{A}} p(s,a) P(Z_2 \leq y | s, a) \; ds da = F_{Y_2}(y)
\end{equation}
\end{proof}

\begin{lemma}
$\forall \gamma \in [0, 1), \forall Z_1, Z_2: \; Z_1 \preccurlyeq Z_2 \Rightarrow \gamma Z_1 \preccurlyeq \gamma Z_2$
\end{lemma}
Can be simply shown via definition.

\textbf{Definition.} Let us remind the notation introduced in section \ref{subsec:unbiasedness}.

Distributional Bellman operator $\mathcal{T}^{\pi}$:
\begin{equation}
    [\mct^\pi Z](s,a) \buildrel d \over = R(s, a) + \gamma Z(s', a')
\end{equation}
$$
\text{where} \quad s' \sim p_{\text{env}}(\cdot|s,a), \quad a' \sim \pi(\cdot|s').
$$

Truncated version: $\mct^{\pi, \eta} = \mct^\pi \circ \mcs^\eta$.


\begin{lemma}
$Z_1 \preccurlyeq Z_2 \Rightarrow \mct^\pi Z_1 \preccurlyeq \mct^\pi Z_2$
\end{lemma}
Follows from the previous three lemmas.


Consider supremum norm of action-value functions:
    $||Q||_\infty = \sup_{s, a} |Q(s,a)|$

\begin{lemma}
$||\ex_z \mct^\pi Z - Q^\pi||_\infty \leq \gamma ||\ex_z Z - Q^\pi||_\infty$
\end{lemma}
\begin{proof}
\begin{equation}\label{eq:27}
\forall s, a \quad |\ex_z \mct^\pi Z(s, a) - Q^\pi(s,a)| = 
\end{equation}

\begin{equation}
    |\ex_{s', r \sim p_\text{env}(s,a)} \ex_{a' \sim \pi(s')} \left[ r + \gamma \ex_z Z(s', a') \right] -  \ex_{s', r \sim p_\text{env}(s,a)} \ex_{a' \sim \pi(s')} \left[ r + \gamma Q^\pi(s', a') \right]| =
\end{equation}

\begin{equation}
    \gamma |\ex_{s' \sim p_\text{env}(s,a)} \ex_{a' \sim \pi(s')}  [\ex_z Z(s', a') - Q^\pi(s', a')]| \leq 
\end{equation}

\begin{equation}
    \gamma \sup_{s, a} |\ex_z Z(s, a) - Q^\pi(s,a)| = \gamma ||\ex_z Z - Q^\pi||_\infty
\end{equation}

Applying supremum to left-hand side we get:

\begin{equation}
    ||\ex_z \mct^\pi Z - Q^\pi||_\infty = \sup_{s,a} |\ex_z \mct^\pi Z(s, a) - Q^\pi(s,a)|  \leq \gamma ||\ex_z Z - Q^\pi||_\infty
\end{equation}
\end{proof}

Now lets consider policy evaluation process with truncation $Z_{t+1} = T^{\pi, \eta} Z_t$ for fixed $\pi, \eta$. Also denote sequence without truncation $Z_{t+1}^0 = \mct^{\pi, 0}Z_t^0 = \mct^{\pi}Z_t^0$. Both these sequences start in the same starting point $Z_0$.

Lemma 10 shows that sequence $\ex_z Z_t^0$ exponentially fast and uniformly on $s, a$ converges to $Q^\pi$, therefore

\begin{equation}\label{eq:upper_limit}
    \forall \varepsilon > 0\; \exists t_1: \forall t' > t_1 : \sup_{s,a} |\ex_z Z_{t'}(s,a) - Q^\pi(s,a)| \leq \varepsilon
\end{equation}

\begin{lemma}
\begin{equation}\label{eq:z_inequality}
    \forall s, a, t \quad \ex_z Z_t(s,a) \leq \ex_z Z_t^0(s,a)
\end{equation}
\end{lemma}

It follows from lemmas 1, 4, 8 and the fact that both sequences have the same starting point.

% We can see that 

% $$\ex Z_t^0 = \ex (T^{\pi, 0})^t Z_0 \rightarrow_{uniformly s, a}^{t \rightarrow \infty} Q^\pi$$


% $$\forall \varepsilon \quad \exists t_1: \forall t' > t_1 :$$
%     $$\sup_{s,a} |\ex Z^0_{t'}(s,a) - Q^\pi(s,a)| \leq \varepsilon$$
%     \begin{equation}\label{eq:upper_limit}
%         \forall s, a \quad \ex Z^0_{t'}(s,a) \leq Q^\pi(s,a) + \varepsilon
%     \end{equation}
    
Let's denote probability density $\hat{p}(s', a')$ based on probability distribution $p_\text{agg}(s)$ considered in section \ref{subsec:bias_est}:
\begin{equation}
    \hat{p}(s', a') = \ex_{s \sim p_\text{agg}} \ex_{a \sim \pi(s)} p_\text{env}(s'|s,a) \pi(a'|s')
\end{equation}
    
\textbf{Definition.} Let's define $Z_t$ "sufficiently stochastic" for fixed $\eta, \pi$ if $\exists \alpha(\eta) > 0$
$$ \ex_{s', a' \sim \hat{p}} \left[\ex_z \mcs^{\eta} Z_t(s',a') - \ex_z Z_t(s',a') \right] \leq - \alpha(\eta) $$


\paragraph{Intuition} Sufficient stochasticity is a property of an environment and a policy.
It states that there are enough state-action pairs, where truncation leads to a non-negligible decrease in the expected value of a distribution over returns. 
During training, our stochastic policy is explicitly encouraged to have non-zero entropy.
That, together with long trajectories lead to the sufficiently stochastic distribution over returns. 
In other words, we speculate that sufficient stochasticity is quite a weak requirement, and is often satisfied in practice.

\begin{theorem_proof}
Lets assume, that we evaluate policy by sequentially applying truncated distributional Bellman operator $Z_{t+1} = \mathcal{T}^{\pi, \eta} Z_{t}$ to some initial random field $Z_0$ and that starting from some moment sequence $Z_t$ becomes sufficiently stochastic:

$$\exists t_2, \alpha(\eta): \forall t' > t_2$$
$$\ex_{s', a' \sim \hat{p}} \left[\ex_z \mcs^{\eta} Z_t(s',a') - \ex_z Z_t(s',a') \right] \leq - \alpha(\eta)$$

Then $\exists t_3, \kappa > 0: \forall t' > t_3$
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)} \left[ \ex_z Z_{t'}(s,a) - Q^\pi(s,a) \right] \leq -\kappa$$

\end{theorem_proof}
\begin{proof}
Lets take $\varepsilon = \alpha(\eta)\gamma/2$ in \ref{eq:upper_limit}. Then take $t' \geq \max(t_1, t_2)$.

$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)} \ex_z Z_{t'+1}(s,a) = $$

$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  \ex_z \mct^{\pi, \eta} Z_{t'}(s,a) =$$
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  \ex_{r, s', a'} [r + \gamma \ex_z \mcs^{\eta}  Z_{t'}(s', a')] \leq $$
sufficient stochasticity
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  \ex_{r, s', a'} [r + \gamma \ex_z  Z_{t'}(s', a')] -\gamma \alpha(\eta) =$$
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  \ex_z \mct^{\pi, 0} Z_{t'}(s,a) - \gamma \alpha(\eta) \leq $$
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  \ex_z \mct^{\pi, 0} Z_{t'}^0(s,a) - \gamma \alpha(\eta) = $$
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  \ex_z Z_{t'+1}^0(s,a)  - \gamma \alpha(\eta) \leq $$
equation \ref{eq:upper_limit}
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  Q^\pi(s,a)  - \gamma \alpha(\eta) + \dfrac{\gamma\alpha(\eta)}{2} = $$
$$\ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)}  Q^\pi(s,a)  - \dfrac{\gamma\alpha(\eta)}{2}$$

We get that
\begin{equation}
    \ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)} \ex_z Z_{t'+1}(s,a) \leq \ex_{s \sim p_{\text{agg}}} \ex_{a \sim \pi(s)} Q^\pi(s,a)  - \dfrac{\gamma\alpha(\eta)}{2}
\end{equation}

The theorem has been proven with $t_3 = \max(t_1, t_2) + 1$, $\kappa = \dfrac{\gamma\alpha(\eta)}{2}$.
\end{proof}

\textbf{Understanding~} The theorem, in other words, means that during an evaluation of a fixed policy with \emph{truncated distributional Bellman} operator and a constant~$\eta$, staring from some point, the measured aggregated bias will be negative.
Effectively leading to a decrease of $\eta$ at optimization steps.
\newline
\newline
In practice, we expect that if $\eta$ changes slowly enough it will converge to zero ($\eta \rightarrow 0$), leading to an unbiased policy evaluation ($\mathcal{T}^{\pi, \eta} \rightarrow \mathcal{T}^{\pi}$, $\mathbb{E}_z Z_t \rightarrow Q^\pi$). We support this hypothesis empirically, on a DNN-based model and real optimization trajectories (Figure \ref{fig:fixed_policy}).
